Exploration of Large Networks with Covariates via Fast and Universal Latent Space Model Fitting

Latent space models are effective tools for statistical modeling and exploration of network data. These models can effectively model real world network characteristics such as degree heterogeneity, transitivity, homophily, etc. Due to their close connection to generalized linear models, it is also natural to incorporate covariate information in them. The current paper presents two universal fitting algorithms for networks with edge covariates: one based on nuclear norm penalization and the other based on projected gradient descent. Both algorithms are motivated by maximizing likelihood for a special class of inner-product models while working simultaneously for a wide range of different latent space models, such as distance models, which allow latent vectors to affect edge formation in flexible ways. These fitting methods, especially the one based on projected gradient descent, are fast and scalable to large networks. We obtain their rates of convergence for both inner-product models and beyond. The effectiveness of the modeling approach and fitting algorithms is demonstrated on five real world network datasets for different statistical tasks, including community detection with and without edge covariates, and network assisted learning.

==> kernel.tex <==
%!TEX root = main.tex
\section{Proof for a Kernel Matrix}
\subsection{Convex Part}
\begin{assumption}
The \emph{stable rank} of the covariate matrix $\bX$ satisfies $\srank(\bX)=\fro{X}^2/\op{X}^2\geq M_0 k$ for some large enough constant $M_0$. 
 \label{assump:kernel-srank}
\end{assumption}
\begin{lemma}
For any $Z\in\mathbb{R}^{n\times k}$, define $\mathcal{M}^\perp_k=\Big\{\bM\in\mathbb{R}^{n\times n}\big| row(\bM)\subset col(Z^{\perp}), col(\bM)\subset col(Z^{\perp})\Big\}$ and $\mathcal{M}_k=\left(\mathcal{M}^{\perp}_k \right)^{\perp}$. Then, if $\lambda_n\geq 2\op{A-P}$
\begin{equation}
\begin{aligned}
\|\dg \|_* \leq 4\sqrt{2k}\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + 2\fro{\da\one^\top}+ \frac{2}{\lambda_n}|\big \langle \bA-\bP, \db\bX \big\rangle| + 2\| \gbar\|_*
\end{aligned}
\end{equation}
\label{lem:kernel-cone}
\end{lemma}
\begin{proof}
	Let $\wl (\bTheta)=-\sum_{i, j}\left\{ \bA_{ij}\bTheta_{ij} + \log\Big(1-\sigma(\bTheta_{ij})\Big)\right\}$. Due to the convexity of $\wl (\bTheta)$,
\begin{equation}
\begin{aligned}
\wl(\hbTheta)-\wl(\bTheta)&\geq  \big \langle \nabla_{\bTheta} \wl(\tall), \dall \big\rangle\\
& = \big\langle  \bA-\bP,\dg+2 \da\one^\top +\dbt\bX \big\rangle\\
&\geq  -\op{\bA-\bP}\Big(\|\dg\|_*+2\|\da\one^\top\|_*\Big) - |\big \langle  \bA-\bP, \db\bX \big\rangle|\\
&\geq -\frac{\lambda_n}{2}\Big(\|\mathcal{P}_{\mathcal{M}_k}\dg\|_*+\|\mathcal{P}_{\mathcal{M}^\perp_k}\dg\|_*+2\fro{\da\one^\top}\Big) - |\big \langle  \bA-\bP, \db\bX \big\rangle|
\nonumber
\end{aligned}
\end{equation}
On the other hand, 
\begin{equation}
\begin{aligned}
\|\hbG\|_*-\|\tg\|_*&=\|\mathcal{P}_{\mathcal{M}_k}\tg+ \gbar++\mathcal{P}_{\mathcal{M}_k}\dg+\mathcal{P}_{\mathcal{M}^\perp_k}\dg\|_*-\|\mathcal{P}_{\mathcal{M}_k}\tg+ \gbar\|_*\\
&\geq \|\mathcal{P}_{\mathcal{M}_k}\tg+\mathcal{P}_{\mathcal{M}^\perp_k}\dg\|_* -\|\gbar\|_*-\|\mathcal{P}_{\mathcal{M}_k}\dg\|_* - \|\mathcal{P}_{\mathcal{M}_k}\tg\|_*- \|\gbar\|_*\\
&=\|\mathcal{P}_{\mathcal{M}_k}\tg\|_*+\|\mathcal{P}_{\mathcal{M}^\perp_k}\dg\|_* - 2\|\gbar\|_* - \|\mathcal{P}_{\mathcal{M}_k}\dg\|_* - \|\mathcal{P}_{\mathcal{M}_k}\tg\|_* \\
&=\|\mathcal{P}_{\mathcal{M}^\perp_k}\dg\|_*-\|\mathcal{P}_{\mathcal{M}_k}\dg\|_* - 2\|\gbar\|_*
\end{aligned}
\end{equation} 
The second line is by triangle inequality and the third line is because $\bG^*$ and $\mathcal{P}_{\mathcal{M}^\perp_k}$ has perpendicular column and row space. Notice that $\hbTheta=\hbalpha\one^\top+\one\hbalpha^\top+\hbeta\bX+\hbG$ is the optimal solution of \eqref{eq:convex-obj}, and $\tall=\ta\one^\top+\one\ta^\top+\tb\bX+\tg$ belongs to the feasible set, then
\begin{equation}
\begin{aligned}
0 &\geq \wl (\hbTheta) - \wl (\tall)+\lambda_n\left( \|\hbG\|_* - \|\tg\|_*\right)\\
&\geq -\frac{\lambda_n}{2}\Big(\|\mathcal{P}_{\mathcal{M}_k}\dg\|_*+\|\mathcal{P}_{\mathcal{M}^\perp_k}\dg\|_*+2\fro{\da\one^\top}\Big)\\
&\quad\quad\quad\quad\quad - |\big \langle  \bA-\bP, \db\bX \big\rangle| + \lambda_n\Big(\|\mathcal{P}_{\mathcal{M}^\perp_k}\dg\|_*-\|\mathcal{P}_{\mathcal{M}_k}\dg\|_* - 2\|\gbar\|_*\Big)\\
&\geq \frac{\lambda_n}{2} \Big(\|\mathcal{P}_{\mathcal{M}^\perp_k}\dg\|_*- 3\|\mathcal{P}_{\mathcal{M}_k}\dg\|_*  - 2\|\gbar\|_* - 2\fro{\da\one^\top}\Big)- |\big \langle  \bA-\bP, \db\bX \big\rangle|
\end{aligned}
\end{equation}
Therefore,
\begin{equation}
\|\mathcal{P}_{\mathcal{M}^\perp_k}\dg \|_* \leq 3\|\mathcal{P}_{\mathcal{M}_k}\dg \|_* + 2\fro{\da\one^\top}  + \frac{2}{\lambda_n}|\big \langle \bA-\bP, \db\bX \big\rangle| + 2\|\gbar\|_*
\end{equation}
and by triangle inequality, 
\begin{equation}
\|\dg \|_* \leq 4\|\mathcal{P}_{\mathcal{M}_k}\dg \|_* + 2\fro{\da\one^\top}+ \frac{2}{\lambda_n}|\big \langle \bA-\bP, \db\bX \big\rangle| + 2\|\gbar\|_*
\end{equation}
Finally, notice that $\mathcal{P}_{\mathcal{M}_k}\dg=\mathcal{P}_{Z}\dg+\dg\mathcal{P}_{Z}-\mathcal{P}_{Z}\dg\mathcal{P}_{Z}=ZZ^\top\dg+\dg ZZ^\top-ZZ^\top\dg ZZ^\top=ZZ^\top\dg(\bI-ZZ^\top)+\dg ZZ^\top$, the rank of $\mathcal{P}_{\mathcal{M}_k}\dg$ is at most $2k$ which implies, 
\begin{equation}
\|\dg \|_* \leq 4\sqrt{2k}\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + 2\fro{\da\one^\top}+ \frac{2}{\lambda_n}|\big \langle \bA-\bP, \db\bX \big\rangle| + 2\|\gbar\|_*
\end{equation}
\end{proof}

\begin{lemma} 
If Assumption~\ref{assump:srank} holds, there exist constants $C_1, C_2$ and $0\leq c<1$  such that either 
\begin{equation}
\begin{gathered}
 \fro{\dall}^2 \geq (1 - c)\left(\fro{\dg}^2 + 2\fro{\da\one^\top}^2+\fro{\db\bX}^2\right) - C\|\gbar\|_*^2/k \\
\fro{\dall}^2\leq (1 + c) \left(\fro{\dg}^2 + 2\fro{\da\one^\top}^2+\fro{\db\bX}^2\right) + C\|\gbar\|_*^2/k 
\end{gathered}
\end{equation}
\label{lem:kernel-identifiability}
\end{lemma}
\begin{proof}
	\begin{equation}
\begin{aligned}
\fro{\dall}^2&=\fro{\dg+\da\one^\top+\one\da^\top+\db\bX}^2\\
&=\fro{\dg+\da\one^\top+\one\da^\top}^2+\fro{\db X}^2+2\big\langle \dg+\da\one^\top+\one\da^\top, \db\bX \big\rangle\\
&=\fro{\dg}^2+2\fro{\da\one^\top}^2+2tr(\da\one^\top\da\one^\top)+\fro{\db X}^2\\
&\quad\quad+2\big\langle \dg+2\da\one^\top, \db\bX \big\rangle
\end{aligned}
\nonumber
\end{equation}
where the last equality is due to the symmetry of $\bX$. Notice that $\,tr(\da\one^\top\da\one^\top)=tr(\one^\top\da\one^\top\da)=|\one^\top\da|^2\geq 0$, 
\begin{equation}
\begin{aligned}
\fro{\dall}^2&\geq \fro{\dg}^2+2\fro{\da\one^\top}^2+\fro{\db X}^2+2\big\langle \dg+2\da\one^\top, \db\bX \big\rangle
\end{aligned}
\label{identi-obj}
\end{equation}
By Holder's inequality, $|\big\langle \dg, \db\bX \big\rangle|\leq \|\dg\|_*\op{\db\bX}$ and further apply Lemma~\ref{lem:kernel-cone}, 
\begin{equation}
\begin{aligned}
|\big\langle \dg +2\da\one^\top &, \db\bX \big\rangle|\leq \Big(4\sqrt{2k}\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + 4\fro{\da\one^\top}+ \frac{2}{\lambda_n}|\big \langle \bA-\bP, \db\bX \big\rangle| + 2\|\gbar\|_*\Big)\op{\db\bX}\\
&\leq \Big(4\sqrt{2k}\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + 4\fro{\da\one^\top}+ 2\sqrt{k}\fro{\db\bX} + 2\|\gbar\|_* \Big)\fro{\db X}/\sqrt{\srank(\bX)}\\
& \leq \frac{C_0\sqrt{k}}{\sqrt{\srank(\bX)}} \left(\fro{\dg}^2+2\fro{\da\one^\top}^2+\fro{\db\bX}^2\right) + \frac{2\|\gbar\|_*}{\sqrt{\srank(\bX)}} \fro{\db X}\\
& \leq \frac{C_0\sqrt{k}}{\sqrt{\srank(\bX)}} \left(\fro{\dg}^2+2\fro{\da\one^\top}^2+\fro{\db\bX}^2\right) + \frac{\|\gbar\|_*^2}{c_0\srank(\bX)} + c_0\fro{\db X}^2
\end{aligned}
\nonumber
\end{equation}
for any constant $c_0\geq 0$.  
% \begin{equation}
% 	\|\gbar\|_* \leq C_1\sqrt{k} \left(\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + \fro{\da\one^\top} + \fro{\db\bX}\right),
% \end{equation}
% then 
% \begin{equation}
% \begin{aligned}
% 	|\big\langle \dg +2\da\one^\top, \db\bX \big\rangle| &\leq  C_2\sqrt{k} \left(\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + \fro{\da\one^\top} + \fro{\db\bX}\right)\op{\db\bX}\\
% 	&\leq C_2\sqrt{k} \left(\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + \fro{\da\one^\top} + \fro{\db\bX}\right)\fro{\db X}/\sqrt{\srank(\bX)}\\
% 	& \leq \frac{C_3\sqrt{k}}{\sqrt{\srank(\bX)}} \left(\fro{\dg}^2+2\fro{\da\one^\top}^2+\fro{\db\bX}^2\right)
% \end{aligned}
% \end{equation}
Substitute these inequalities into \eqref{identi-obj}, 
\begin{equation}
\begin{aligned}
\fro{\dall}^2 & \geq \left(1-\frac{2C_0\sqrt{k}}{\sqrt{\srank(\bX)}} \right)\fro{\dg}^2 + \left(2 - \frac{2C_0\sqrt{k}}{\sqrt{\srank(\bX)}}\right)\fro{\da\one^\top}^2\\
&\quad\quad+\left(1 - \frac{2C_0\sqrt{k}}{\sqrt{\srank(\bX)}} - 2c_0 \right)\fro{\db X}^2 - \frac{2\|\gbar\|_*^2}{c_0\srank(\bX)}
\end{aligned}
\nonumber
\end{equation}
On the other hand, notice that $tr(\da\one^\top\da\one^\top)\leq \|\da\one\|_F^2$, we have
\begin{equation}
\begin{aligned}
\fro{\dall}^2&\leq \left(1 + \frac{2C_0\sqrt{k}}{\sqrt{\srank(\bX)}}  \right)\fro{\dg}^2+\left(4 + \frac{2C_0\sqrt{k}}{\sqrt{\srank(\bX)}} \right)\fro{\da\one^\top}^2\\
&\quad\quad+\left(1 + \frac{2C_0\sqrt{k}}{\sqrt{\srank(\bX)}} + 2c_0  \right)\fro{\db X}^2 + \frac{2\|\gbar\|_*^2}{c_0\srank(\bX)}
\end{aligned}
\nonumber
\end{equation}
% Else if 
% \begin{equation}
% 	\|\gbar\|_* \geq C_1\sqrt{k} \left(\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + \fro{\da\one^\top} + \fro{\db\bX}\right),
% \end{equation}
% then 
% \begin{equation}
% \begin{aligned}
% 	|\big\langle \dg +2\da\one^\top, \db\bX \big\rangle| &\leq \left(1 + C_1^{-1}\right) \|\gbar\|_*\op{\db\bX}\\
% 	&\leq \left(1 + C_1^{-1}\right) \|\gbar\|_*\fro{\db X}/\sqrt{\srank(\bX)}\\
% 	& \leq 2 \|\gbar\|_*^2/\sqrt{k\srank(\bX)}。
% \end{aligned}
% \end{equation}
% Therefore, 
% \begin{equation}
% \begin{aligned}
% \fro{\dall}^2&\leq \fro{\dg}^2+4\fro{\da\one^\top}^2+\fro{\db X}^2+2\big\langle \dg+2\da\one^\top, \db\bX \big\rangle\\
% &\leq C_4\|\gbar\|_*^2/k
% \end{aligned}
% \end{equation}
\end{proof}




\begin{theorem}(Deterministic Bound)
Choose any $\lambda_n$ such that $\lambda_n\geq \max\{2\op{\bA-\bP}, 1\}$ and $| \langle \bA-\bP, \bX \rangle | \leq \lambda_n \sqrt{k}\fro{X}$, under Assumption~\ref{assump:srank}, there exists a constant $C$ such that
\begin{equation}
\fro{\dall}^2\leq C\left(\frac{\lambda_n^2k}{\tau^2} + \frac{\lambda_n \|\gbar\|_*}{\tau}\right)
\nonumber
\end{equation}
where $\tau=e^M/(1+e^M)^2$.
\label{thm:kernel-upper-deter}
\end{theorem} 

\begin{proof}
According to Lemma~\ref{lem:kernel-identifiability}, we only need to consider the case 
\begin{equation}
\begin{gathered}
 \fro{\dall}^2 \geq C_1\|\gbar\|_*^2/k, \\
(1 - c) \leq \fro{\dall}^2/\left(\fro{\dg}^2 + 2\fro{\da\one^\top}^2+\fro{\db\bX}^2\right) \leq (1 + c).
\end{gathered}
\label{eq:kernel-second-case}
\end{equation}
	Let $\wl (\bTheta)=-\sum_{i, j}\left\{ \bA_{ij}\bTheta_{ij}+log\Big(1-\sigma(\bTheta_{ij})\Big)\right\}$. Observe that $\hbTheta=\hbalpha\one^\top+\one\hbalpha^\top+\hbeta\bX+\hbG$ is the optimal solution of \eqref{eq:convex-obj}, and the true parameter $\tall=\ta\one^\top+\one\ta^\top+\tb\bX+\tg$ is a feasible solution, then
\begin{equation}
\wl(\hbTheta)-\wl(\tall)+\lambda_n \left(\|\hbG\|_*-\|\tg\|_*\right)\leq 0
\nonumber
\end{equation}
For $\bTheta\in\mathcal{F}(n, k, M, \bX)$, 
$$\nabla^2 \wl(\bTheta)=diag\Big(vec\big(\sigma(\bTheta) \circ \left(1-\sigma(\bTheta)\right)\big)\Big)\succeq \tau\bI_{n^2\times n^2}$$
where $\tau=e^M/(1+e^M)^2$, then by Taylor expansion, 
\begin{equation}
\wl(\hbTheta)-\wl(\tall)\geq \big\langle \nabla_{\bTheta} \wl(\tall),\dall \big\rangle +\frac{\tau}{2}\fro{\dall}^2
\nonumber
\end{equation}
On the other hand, by triangular inequality
\begin{equation}
\lambda_n \left(\|\hbG\|_*-\|\tg\|_*\right)\geq -\lambda_n\|\Delta_{\bG}\|_*
\nonumber
\end{equation}
Combine the inequalities above, 
\begin{equation}
\big\langle \nabla_{\bTheta} \wl (\tall),\dall \big\rangle +\frac{\tau}{2}\fro{\dall}-\lambda_n\|\dg\|_*\leq 0
\nonumber
\end{equation}
Manipulate by simple algebra,
\begin{equation}
\begin{aligned}
\frac{\tau}{2}\|\Delta_{\bTheta}\|_F^2&\leq \lambda_n\|\Delta_{\bG}\|_*
+\left|\big\langle \nabla_{\bTheta} \wl (\tall),\dg+ \da\one^\top +\one\da^\top  \big\rangle\right|
 +\left|\db\big\langle \nabla_{\bTheta} \wl(\tall), \bX \big\rangle\right|\\
 &=\lambda_n\|\Delta_{\bG}\|_*
+ \left|\big\langle \bA-\bP, \dg+ 2\da\one^\top \big\rangle\right|
 +  \left|\db\big\langle \bA-\bP, \bX \big\rangle\right|\\
 &\leq \lambda_n\|\Delta_{\bG}\|_*
+ \left|\big\langle \bA-\bP, \dg+ 2\da\one^\top \big\rangle\right|
 + \lambda_n\sqrt{k}\fro{\db X}
\end{aligned}
 \label{convexity}
\end{equation}
where the equality is due to the symmetry of $\bA-\bP$. By Holder's inequality, 
\begin{equation}
\begin{aligned}
\left|\big\langle  \bA-\bP,\dg+2 \da\one^\top  \big\rangle\right| &\leq  \op{\bA-\bP}\left(\|\dg\|_*+2\|\da\one^\top\|_*\right)\\
& =\op{\bA-\bP}\left(\|\dg\|_*+2\fro{\da\one^\top}\right)\\
&\leq \frac{\lambda_n}{2}\left(\|\dg\|_*+2\fro{\da\one^\top}\right)
\end{aligned}
\label{eq:kernel-part1}
\end{equation}
By Lemma~\ref{cone-condition} and the assumption that $\left|\big\langle \bA-\bP, \bX \big\rangle\right|\leq \lambda_n\sqrt{k}\fro{X}$,
\begin{equation}
\begin{aligned}
\|\Delta_{\bG}\|_*&\leq 4\sqrt{2k}\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + 2\fro{\da\one^\top}+ 2\sqrt{k}\fro{\db X} + 2\|\gbar\|_*. 
% \\&\leq C_1 \|\gbar\|_*
\end{aligned}
\label{eq:kernel-part2}
\end{equation}
Substitute \eqref{eq:kernel-part1} and \eqref{eq:kernel-part2} into \eqref{convexity}, 
\begin{equation}
\begin{aligned}
\frac{\tau}{2}\fro{\dall}^2 &\leq \frac{3\lambda_n}{2}\|\dg\|_*+\lambda_n \fro{\da\one^\top}+\lambda_n\sqrt{k}\fro{\db X}\\
&\leq \frac{3\lambda_n}{2}\Big(4\sqrt{2k}\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + 2\fro{\da\one^\top}+ 2\sqrt{k}\|\db \bX\|_F + 2\|\gbar\|_*\Big)\\
&\qquad\qquad\qquad\qquad\qquad\qquad\quad+\lambda_n \fro{\da\one^\top}+\lambda_n\sqrt{k}\fro{\db X}\\
& \leq C_1\lambda_n \Big\{\sqrt{k} \Big(\fro{\mathcal{P}_{\mathcal{M}_k}\dg} + \fro{\da\one^\top} + \|\db \bX\|_F \Big) +  \|\gbar\|_* \Big\} \\
&\leq C_2\lambda_n \sqrt{k} \left(\fro{\dall} + \|\gbar\|_* /\sqrt{k} \right) + C_1\lambda_n \|\gbar\|_*\\
&\leq C_2\lambda_n \sqrt{k} \fro{\dall} + (C_1 + C_2)\lambda_n \|\gbar\|_*
\end{aligned}
\end{equation}
Solve this quadratic inequality, 
\begin{equation}
\fro{\dall}^2 \leq C\left(\frac{\lambda_n^2k}{\tau^2} + \frac{\lambda_n \|\gbar\|_*}{\tau}\right).
\end{equation}
\end{proof}

\begin{theorem}
Choose any $\lambda_n$ such that $\lambda_n\geq \max\{2\op{\bA-\bP}, 1\}$ and $| \langle \bA-\bP, \bX \rangle | \leq \lambda_n \sqrt{k}\fro{X}$, under Assumption~\ref{assump:srank}, if $(\tg)_{ij} = f(x_i, x_j)$ for some Lipchitz continuous function $f(\cdot, \cdot)$ and $x_1, \cdots, x_n\in\mathcal{K}$ where $\mathcal{K}$ is a compact set in $\mathbb{R}^r$, then there exists a constant $C$ such that
\begin{equation}
\fro{\dall}\leq C\frac{\lambda_n}{\tau} \max\left\{ 1, \left(\frac{n^{\frac{3}{2}}\tau}{\lambda_n}\right)^{\frac{r}{2(r+1)}} \right\}
\nonumber
\end{equation}
where $\tau=e^M/(1+e^M)^2$.
\label{thm:latent-upper-deter}
\end{theorem} 
\begin{proof}
	By Theorem~\ref{thm:kernel-upper-deter}, \begin{equation}
\fro{\dall}\leq C \left(\lambda_n\sqrt{k}/\tau + \|\gbar\|_*/\sqrt{k}\right) 
\nonumber
\end{equation}
\end{proof}

\subsection{Non-convex Part}
\begin{equation}
e_t=\op{\tz}^2\fro{\dzt}^2+2\fro{\dat\one^\top}^2+\fro{\dbt X}^2.
\end{equation}
\begin{lemma} 
If Assumption~\ref{assump:srank} holds, there exist constants $0\leq c_0<1$ and $C_0$  such that  
\begin{equation}
\begin{gathered}
\fro{\dallt}^2  \geq (1 - c_0)\left(\frac{\kappa^2_{\tz}}{2(\sqrt{2}-1)}\fro{Z^t(Z^t)^\top - ZZ^\top}^2+2\fro{\dat\one^\top}^2+\fro{\dbt X}^2\right) - C_0\fro{\gbar}^2, \\
\fro{\dallt}^2  \leq (1 + c_0)\left(\frac{\kappa^2_{\tz}}{2(\sqrt{2}-1)}\fro{Z^t(Z^t)^\top - ZZ^\top}^2+2\fro{\dat\one^\top}^2+\fro{\dbt X}^2\right) + C_0\fro{\gbar}^2. 
\end{gathered}
\nonumber
\end{equation}
\label{lem:kernel-identifiability-nonconvex}
\end{lemma}
\begin{proof}
By definition,
\begin{equation}
\begin{aligned}
\fro{\dgt}^2 &= \fro{Z^t(Z^t)^\top - ZZ^\top - \widebar{G}}^2\\
& \geq \fro{Z^t(Z^t)^\top - ZZ^\top}^2 + \fro{\widebar{G}}^2 - 2| \big\langle Z^t(Z^t)^\top - ZZ^\top, \widebar{G} \big\rangle|\\
& \geq \fro{Z^t(Z^t)^\top - ZZ^\top}^2 + \fro{\widebar{G}}^2 - 2\fro{Z^t(Z^t)^\top - ZZ^\top}\fro{\widebar{G}}\\
&\geq \fro{Z^t(Z^t)^\top - ZZ^\top}^2 + \fro{\widebar{G}}^2 - c_1\fro{Z^t(Z^t)^\top - ZZ^\top}^2 - c_1^{-1}\fro{\widebar{G}}^2\\
&\geq (1-c_1)\fro{Z^t(Z^t)^\top - ZZ^\top}^2 - (c_1^{-1}-1)\fro{\widebar{G}}^2
\end{aligned}
\end{equation}
where the second last inequality comes from $a^2 + b^2\geq 2ab$ and holds for any $c_1\geq 0$. Similarly, it could be shown that 
\begin{equation}
	\fro{\dgt}^2\leq (1+c_1)\fro{Z^t(Z^t)^\top - ZZ^\top}^2 + (1 + c_1^{-1})\fro{\widebar{G}}^2
\end{equation}
Expand the term $\fro{\dallt}^2$,
\begin{equation}
\begin{aligned}
\fro{\dallt}^2&=\fro{\dgt+\dat\one^\top+\one\dat^\top+\dbt\bX}^2\\
&=\fro{\dgt+\dat\one^\top+\one\dat^\top}^2+\fro{\dbt X}^2+2\big\langle \dgt+\dat\one^\top+\one\dat^\top, \dbt\bX \big\rangle\\
&=\fro{\dgt}^2+2\fro{\dat\one^\top}^2+2tr(\dat\one^\top\dat\one^\top)+\fro{\dbt X}^2\\
&\quad\quad+2\big\langle \dgt+2\dat\one^\top, \dbt\bX \big\rangle
\end{aligned}
\nonumber
\end{equation}
where the last equality is due to the symmetry of $\bX$. Notice that $\,tr(\da\one^\top\da\one^\top)=tr(\one^\top\da\one^\top\da)=|\one^\top\da|^2\geq 0$, 
\begin{equation}
\begin{aligned}
\fro{\dallt}^2&\geq (1-c_1)\fro{Z^t(Z^t)^\top - ZZ^\top}^2 - (c_1^{-1}-1)\fro{\widebar{G}}^2+2\fro{\dat\one^\top}^2+\fro{\dbt X}^2\\
&\quad+2\big\langle Z^t(Z^t)^\top - ZZ^\top +  2\dat\one^\top, \dbt\bX \big\rangle - 2\inner{\gbar, \dbt\bX }
\end{aligned}
\label{identi-obj}
\end{equation}
By Holder's inequality,
\begin{equation}
\begin{aligned}
|\big\langle Z^t(Z^t)^\top - ZZ^\top &+  2\dat\one^\top, \dbt\bX \big\rangle|\leq \left(\|Z^t(Z^t)^\top - ZZ^\top\|_* + 2\|\dat\one^\top\|_* \right)\op{\dbt\bX}\\
&\leq \left( \sqrt{2k}\fro{Z^t(Z^t)^\top - ZZ^\top} + 2\fro{\dat\one^\top}\right)\op{\dbt\bX} \\
&\leq \left( \sqrt{2k}\fro{Z^t(Z^t)^\top - ZZ^\top} + 2\fro{\dat\one^\top}\right)\fro{\dbt\bX}/\sqrt{\srank(X)}\\
&\leq C_1\sqrt{\frac{k}{\srank(X)}}\left(\fro{Z^t(Z^t)^\top - ZZ^\top}^2 + \fro{\dat\one^\top}^2+\fro{\dbt\bX}^2\right)
\end{aligned}
\nonumber
\end{equation}
and for any $c>0$,
\begin{equation}
	|\inner{\gbar, \dbt\bX }| \leq \fro{\gbar}\fro{\dbt\bX} \leq c\fro{\dbt\bX}^2 + \frac{1}{4c}\fro{\gbar}^2. 
\end{equation}
Substitute these inequalities into \eqref{identi-obj}, 
\begin{equation}
\begin{aligned}
\fro{\dall}^2 & \geq \left(1-2C_1\sqrt{\frac{k}{\srank(X)}}-c_1 \right)\fro{Z^t(Z^t)^\top - ZZ^\top}^2 + \left(2 - 2C_1\sqrt{\frac{k}{\srank(X)}}\right)\fro{\dat\one^\top}^2\\
&\quad\quad+\left(1 - 2C_1\sqrt{\frac{k}{\srank(X)}} - 2c \right)\fro{\dbt X}^2 - (c_1^{-1}+1/2c)\fro{\gbar}^2
\end{aligned}
\nonumber
\end{equation}
On the other hand, notice that $tr(\dat\one^\top\dat\one^\top)\leq \|\dat\one\|_F^2$, we have
\begin{equation}
\begin{aligned}
\fro{\dall}^2 & \geq \left(1+2C_1\sqrt{\frac{k}{\srank(X)}}+c_1 \right)\fro{Z^t(Z^t)^\top + ZZ^\top}^2 + \left(2 + 2C_1\sqrt{\frac{k}{\srank(X)}}\right)\fro{\da\one^\top}^2\\
&\quad\quad+\left(1 + 2C_1\sqrt{\frac{k}{\srank(X)}} + 2c \right)\fro{\dbt X}^2 + (c_1^{-1}+1/2c)\fro{\gbar}^2
\end{aligned}
\nonumber
\end{equation}
\end{proof}
 
% \begin{lemma} 
% Let $\kappa_{\tz}$ be the condition number of $\tz$, then
% \begin{equation}
% \begin{aligned}
% e_t &\leq \frac{\kappa^2_{\tz}}{2(\sqrt{2}-1)}\fro{Z^t(Z^t)^\top - ZZ^\top}^2+2\fro{\dat\one^\top}^2+\fro{\dbt X}^2\\
% &\leq \frac{\kappa^2_{\tz}}{2(\sqrt{2}-1)(1-c_1)}\fro{\dgt}^2+2\fro{\dat\one^\top}^2+\fro{\dbt X}^2 + \frac{c_1^{-1}-1}{1-c_1}\fro{\widebar{G}}^2\\
% &\leq  \frac{\kappa^2_{\tz}}{2(\sqrt{2}-1)(1-c_0)(1-c_1)} \left( \fro{\dallt}^2 + 2\|\gbar\|_*^2/k\right)+ \frac{c_1^{-1}-1}{1-c_1}\fro{\widebar{G}}^2
% \end{aligned}
% \end{equation}
% Moreover, if $\text{dist}(\zt, \tz)\leq c\op{\tz}$, we have 
% \begin{equation}
% \begin{aligned}
% e_t &\geq \frac{1}{2+c}\fro{Z^t(Z^t)^\top - ZZ^\top}^2+2\fro{\dat\one^\top}^2+\fro{\dbt X}^2\\
% &\geq \frac{1}{(2+c)(1+c_1)}\fro{\dgt}^2+2\fro{\dat\one^\top}^2+\fro{\dbt X}^2-\frac{1+c_1^{-1}}{1+c_1}\fro{\widebar{G}}^2\\
% &\geq  \frac{1}{(2+c)(1+c_0)(1+c_1)}\left(\fro{\dallt}^2- 2\|\gbar\|_*^2/k\right)-\frac{1+c_1^{-1}}{1+c_1}\fro{\widebar{G}}^2.
% \end{aligned}
% \end{equation}
% \label{error-metric}
% \end{lemma}

\begin{theorem}[Linear Convergence of Algorithm~\ref{alg:non-convex}] 
Under Assumption~\ref{assump:srank}, \ref{assump:constraint}, \ref{assump:init}, there exists constant $c$, for any $\eta\leq c$, and $\op{\tz}^2\geq C_1\kappa_{\tz}^2\lambda_n/\tau\max\left\{\sqrt{\eta\fro{G}^2/\lambda_n^2}, \sqrt{\eta k/\tau}, 1\right\}$, choose step sizes as $\etaz=\eta/\op{\tz}^2, \etaa=\eta/(2n), \etab=\eta/(2\fro{X}^2)$, constraint sets as
$$\projz = \{Z\in\mathbb{R}^{n\times k}, JZ = Z, \max_{1\leq i\leq n}\|Z_{i*}\|\leq M/3\}, $$
$$ \proja = \{\alpha\in\mathbb{R}^n, \|\alpha\|_{\infty}\leq M/3\}, ~\projb = \{\beta\in\mathbb{R}, \beta\|X\|_{\infty} \leq M/3\},$$
and also choose $\lambda_n$ such that $\lambda_n\geq 2  \op{\bA-\bP}$ and $| \langle \bA-\bP, \bX \rangle | \leq \lambda_n \sqrt{k}\fro{X}$. If $\smin^2(\tz)\geq C_1\lambda_n\sqrt{k}/\tau$ for a sufficiently large constant $C_1$, there exist positive constants $\rho$ and $C$ such that 
\begin{equation}
e_{t+1}\leq \left(1- \frac{\eta\tau}{\kappa_{\tz}^2}\rho\right)e_t + \eta C \left(\fro{\gbar}^2 + \frac{\lambda_n^2k}{\tau}\right),
\nonumber
\end{equation}
and so
 \begin{equation}
e_t\leq \bigg(1- \frac{\eta\tau}{\kappa_{\tz}^2}\rho \bigg)^t e_0 + C\kappa_{\tz}^2 \left(\frac{\fro{\gbar}^2 }{\tau}+ \frac{\lambda_n^2k}{\tau^2}\right).
\nonumber
\end{equation}
\end{theorem} 


\begin{lemma}
Choosing $\lambda_n\geq 2\op{A-P}$, $| \langle \bA-\bP, \bX \rangle | \leq \lambda_n \sqrt{k}\fro{\bX}$, if $\fro{\dzt}\leq c_0\tau\op{\tz}/\kappa^2_{\tz}$ and $\op{\tz}^2\geq C_0\kappa_{\tz}^2\lambda_n/\tau$ for sufficiently small constant $c_0$ and sufficiently large constant $C_0$, then under Assumption~\ref{assump:srank}, there exists universal constant $c$ such that, for any $\eta\leq c$, there exists positive constants $\rho$ and $C$, 
\begin{equation}
\begin{aligned}
e_{t+1}&\leq \left(1- \frac{\eta\tau}{\kappa^2}\rho\right)e_t + \eta C \left(\fro{\gbar}^2 + \frac{\lambda_n^2k}{\tau}\right)  
\nonumber
\end{aligned}
\end{equation}
\label{lem:kernel-nonconvex-1}
\end{lemma}

\begin{proof}
Let $\allt=\at\one^\top+\one(\at)^\top+\bt\bX+\zt(\zt)^\top\in \mathcal{F}$, $\bR^t=\arg
\min\limits_{\bR\in\mathbb{R}^{r\times r}, \bR\bR^\top=\bI_r} \fro{\zt-\tz\bR}$, $\widetilde{\bR}^t=\arg
\min\limits_{\bR\in\mathbb{R}^{r\times r}, \bR\bR^\top=\bI_r}\fro{\widetilde{\bZ}_t-\tz\bR}$ and $\dzt=\zt-\tz\bR^t$, then
\begin{equation}
\begin{aligned}
\fro{\bZ^{t+1}-\tz\bR^{t+1}}^2&\leq \fro{\bZ^{t+1}-\tz\widetilde{\bR}^{t+1}}^2\\
&\leq \fro{\widetilde{\bZ}_{t+1}-\tz\widetilde{\bR}^{t+1}}^2 \\
&\leq \fro{ \widetilde{\bZ}_{t+1}-\tz\bR^{t}}^2
\end{aligned}
\end{equation}
The first and last inequality are due to the definition of $\bR^{t+1}$ and $\widetilde{\bR}^{t+1}$, and the second inequality is due to the fact that the rows of $\bZ_{*}\widetilde{\bR}^{t+1}$ have $l_2$ norm less than $M_1$. Plug in the definition of $ \widetilde{\bZ}^{t+1}$, 
\begin{equation}
\begin{aligned}
\fro{\bZ^{t+1}-\tz \bR^{t+1}}^2&\leq \fro{\zt-\tz\bR^{t}}^2+\etaz^2\fro{\samt \zt}^2- 2\etaz\inner{\samt\zt, \zt-\tz\bR^t }\\
&=\fro{\zt-\tz\bR^{t}}^2+\etaz^2\fro{\samt \zt}^2- 2\etaz\inner{\samt, (\zt-\tz\bR^t)(\zt)^\top }
\end{aligned}
\end{equation}
Notice that, 
\begin{equation}
\zt(\zt)^\top-\tz\bR^t(\zt)^\top=\frac{1}{2}(\zt(\zt)^\top-\tz\tz^\top)+\frac{1}{2}(\zt(\zt)^\top+\tz\tz^\top)-\tz\bR(\zt)^\top
\end{equation}
Also due to the symmetry of $\samt$,
\begin{equation}
\inner{\samt , \frac{1}{2}(\zt(\zt)^\top+\tz\tz^\top)-\tz\bR(\zt)^\top}=\frac{1}{2}\inner{\samt, \dzt\dzt^\top}
\end{equation}
Therefore, combine the above three equations,
\begin{equation}
\begin{aligned}
\fro{ \bZ^{t+1}-\tz\bR^{t+1}}^2&\leq \fro{ \zt-\tz\bR^{t}}^2+\etaz^2\fro{\samt \zt}^2-\etaz\inner{\samt , \dzt\dzt^\top} \\
&\quad -\etaz\inner{\samt ,(\zt(\zt)^\top-\tz\tz^\top)}
\end{aligned}
\label{non-convex-obj-Z}
\end{equation}
By similar while much simpler argument, one will obtain
\begin{equation}
\begin{aligned}
\| \balpha^{t+1}-\at\|^2&\leq \|\widetilde{\balpha}_{t+1}-\balpha^{t}\|^2\\
&=\| \balpha^{t}-\ta\|^2+\etaa^2\fro{\samt \one}^2- 2\etaa\inner{\samt\one, \balpha^{t}-\ta}
\end{aligned}
\label{non-convex-obj-a}
\end{equation}
\begin{equation}
\begin{aligned}
\| \beta^{t+1}-\bt\|^2&\leq \|\widetilde{\beta}_{t+1}-\beta^{t}\|^2\\
&=\| \beta^{t}-\tb\|^2+\etab^2\inner{\samt, \bX}^2- 2\etab\inner{\samt, (\beta^{t}-\tb)\bX}
\end{aligned}
\label{non-convex-obj-b}
\end{equation}
Let $\wll (\bTheta)=\E [\,\wl(\bTheta)]$. With $\etaz=\eta/\op{\tz}^2, \etaa=\eta/2n, \etab=\eta/2\fro{X}^2$ , the weighted sum $\op{\tz}^2\times$\eqref{non-convex-obj-Z}+$2n\times$\eqref{non-convex-obj-a}+$\fro{X}^2\times$\eqref{non-convex-obj-b} is equivalent to
\newcommand{\dalltk}{\Delta_{\widebar{\Theta}^t}}
\begin{equation}
\begin{aligned}
e_{t+1}&\leq e_t-\eta\inner{\samt,\dzzt+2(\balpha^{t}-\ta)\one^\top+(\beta^{t}-\tb)\bX+\dzt\dzt^\top}\\
&\quad+\Big(\op{\tz}^2\etaz^2\fro{\samt \zt}^2+2n\etaa^2\fro{\samt \one}^2+\fro{X}^2\etab^2\inner{\samt, \bX}^2 \Big)\\
&= e_t-\eta\inner{\samt-\popt, \dalltk}-\eta\inner{\popt,\dalltk}-\eta\inner{\samt,\dzt\dzt^\top} \\
&\quad+\Big(\frac{\eta^2}{\op{\tz}^2}\fro{\samt \zt}^2+\frac{\eta^2}{2n}\fro{\samt \one}^2+\frac{\eta^2}{4\fro{X}^2}\inner{\samt, \bX}^2 \Big)\\
&= e_t-\eta\inner{\samt - \popt, \dalltk}-\eta\inner{\popt,\dallt}-\eta\inner{\samt,\dzt\dzt^\top} - \eta\inner{\popt,\widebar{G}} \\
&\quad+\Big(\frac{\eta^2}{\op{\tz}^2}\fro{\samt \zt}^2+\frac{\eta^2}{2n}\fro{\samt \one}^2+\frac{\eta^2}{4\fro{X}^2}\inner{\samt, \bX}^2 \Big)\\
&\leq  e_t-\eta\inner{\popt,\dallt}+\eta |\inner{\samt-\popt,\dalltk}| + \eta |\inner{\sam,\dzt\dzt^\top}| + \eta|\inner{\popt,\widebar{G}}| \\
&\quad+\eta^2\Big(\frac{1}{\op{\tz}^2}\fro{\samt \zt}^2+\frac{1}{2n}\fro{\samt \one}^2+\frac{1}{4\fro{X}^2}\inner{\samt, \bX}^2 \Big)\\
&=e_t-\eta\bI_1+\eta\bI_2+\eta\bI_3+\eta I_4+\eta^2\bI_5
\end{aligned}
\label{nonconvex-obj}
\end{equation}
Notice that for $\bTheta\in\mathcal{F}(n, k, M, \bX)$ with $\tau=e^M/(1+e^M)^2$, 
$$\frac{1}{4}\bI_{n^2\times n^2}\succeq \nabla^2 \wll(\bTheta)=diag\Big(vec\big(\sigma(\bTheta)\circ \left(1-\sigma(\bTheta)\right)\big)\Big)\succeq \tau\bI_{n^2\times n^2}$$
Hence $\wll(\cdot)$ is $\tau$-strongly convex and $\frac{1}{4}$-smooth. Further notice that $\popstar=0$, then by Lemma~\ref{lemma-stongly-convex}, 
\begin{equation}
\begin{aligned}
\bI_1=\inner{\popt,\dallt} \geq \frac{\tau/4}{\tau + 1/4}\fro{\dallt}^2 + \frac{1}{\tau+1/4}\fro{\sigt-\sigp}^2
\end{aligned}
\label{nonconvex-I1}
\end{equation}
% By Lemma~\ref{lem:kernel-identifiability-nonconvex}, 
% \begin{equation}
% \begin{aligned}
% 	\bI_1 &\geq \frac{(1-c_1)\tau}{4\tau + 1}\left(\fro{\dzzt}^2+ 2\|\dat\one^\top\|_F^2 +\|\dbt\bX\|_{\rm F}^2 \right) \\
% 	& \quad + \frac{1}{\tau+1/4}\fro{\sigt-\sigp}^2  - C\fro{\gbar}^2	
% \end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
% \bI_1&\geq \frac{\tau}{C_1\kappa^2} e_t + \frac{1}{\tau+1/4}\|\sigt-\sigp\|_F^2 \\
% &\geq \tau(1-c_{M_0})\Big(2(\sqrt{2}-1)\sigma_k^2(\tz)\fro{\dzt}^2+2\fro{\dat\one^\top}^2+\fro{\dbt X}^2\Big)\\
% &\geq \frac{2(\sqrt{2}-1)\tau(1-c_{M_0})}{\kappa^2} e_t
% \end{aligned}
% \end{equation}
% By Lemma~\ref{lemma-tu1}, 
% \begin{equation}
% \begin{aligned}
% \bI_1&\geq  \tau(1-c_{M_0})\Big(2(\sqrt{2}-1)(1-c)\sigma_k^2(\tz)\fro{\dzt}^2+2\fro{\dat\one^\top}^2+\fro{\dbt X}^2\Big) \\
% & ~~~~~~~~~~~~~ - (c^{-1}-1)\fro{\widebar{G}}^2 - 2\tau\|\gbar\|_*^2/k \\
% &\geq \frac{2(\sqrt{2}-1)\tau(1-c_{M_0})(1-c)}{\kappa^2} e_t- (c^{-1}-1)\fro{\widebar{G}}^2 - 2\tau\|\gbar\|_*^2/k
% \end{aligned}
% \end{equation}
By triangle inequality, 
\begin{equation}
\begin{aligned}
\bI_2&\leq |\inner{\sigp - \bA, \dzzt}|+ 2|\inner{\sigp - \bA , \dat\one^\top}| + |\inner{\sigp - \bA , \dbt\bX}|\\
&\leq \frac{\lambda_n}{2} \|\dzzt\|_*  + \lambda_n\|\dat\one^\top\|_*+ \lambda_n\sqrt{k}\fro{\dbt X}\\
&\leq \frac{\lambda_n\sqrt{2k}}{2}\fro{\dzzt}+ \lambda_n\fro{\dat\one^\top} + \lambda_n\sqrt{k}\|\dbt\bX\|_{\rm F} \\
&\leq c_2 \left(\fro{\dzzt}^2 + 2\fro{\dat\one^\top}^2 + \|\dbt\bX\|_{\rm F}^2 \right) + \frac{C_2}{4c_2}\lambda_n^2k
 % \\& \leq C\lambda_n \sqrt{k} \sqrt{e_t} 
\end{aligned}
\end{equation}
for any constant $c_2$ which we will specify later. Then, 
\begin{equation}
\begin{aligned}
I_1 - I_2 &\geq \left(\frac{(1-c_1)\tau}{4\tau + 1} - c_2\right) \left(\fro{\dzzt}^2+ 2\|\dat\one^\top\|_F^2 +\|\dbt\bX\|_{\rm F}^2 \right) \\
	& \quad + \frac{1}{\tau+1/4}\fro{\sigt-\sigp}^2  - C_1\fro{\gbar}^2 - \frac{C_2}{4c_2}\lambda_n^2k	
\end{aligned}
\end{equation}
By Lemma~\ref{lemma-tu1}, 
\begin{equation}
\begin{aligned}
	\bI_1 &\geq \frac{2(\sqrt{2}-1)}{\kappa^2}\left(\frac{(1-c_1)\tau}{4\tau + 1} - c_2\right)e_t  + \frac{1}{\tau+1/4}\fro{\sigt-\sigp}^2  - C_1\fro{\gbar}^2	- \frac{C_2}{4c_2}\lambda_n^2k	
\end{aligned}
\end{equation}
% When $\text{dist}(\zt, \tz)\leq c\op{\tz}$, 
% \begin{equation}
% \begin{aligned}
% I_2 &\leq C_2\lambda_n \sqrt{k} \sqrt{e_t} 
% \end{aligned}
% \end{equation}
% By the inequality $a^2+b^2\geq 2ab$, 
% \begin{equation}
% \begin{aligned}
% \bI_2\leq \frac{c_2}{4\kappa^2} e_t + \frac{C_2^2\kappa^2}{c_2} \lambda_n^2k 
% \end{aligned}
% \label{nonconvex-I2}
% \end{equation}
 To bound $\bI_3$, notice that $\dzt\dzt^\top$ is a positive definite matrix, by von Neumann's trace inequality in Lemma~\ref{lemma-Neumann}, 
\begin{equation}
\begin{aligned}
\bI_3&\leq |\inner{\samt, \dzt\dzt^\top}|\leq \op{\samt}tr(\dzt\dzt^\top)\leq  \op{\samt}\fro{\dzt}^2\\
&=\op{\samt-\popt+\popt}\fro{\dzt}^2\\
&\leq \op{\samt-\popt}\fro{\dzt}^2+\op{\popt}\fro{\dzt}^2\\
&= \op{\sigp-\bA} \fro{\dzt}^2+\op{\sigt-\sigp}\fro{\dzt}^2\\
&\leq \frac{\lambda_n}{2}\fro{\dzt}^2+\fro{\sigt-\sigp}\fro{\dzt}^2
\end{aligned}
\end{equation}
By the assumption that $\fro{\dzt}\leq \frac{c_0\tau}{\kappa^2}\op{\tz}$, 
\begin{equation}
\begin{aligned}
\fro{\sigt-\sigp}\fro{\dzt}^2&\leq \frac{c_0\tau}{\kappa^2}\fro{\sigt-\sigp}\fro{\dzt}\op{\tz}\\
&\leq c_3\fro{\sigt-\sigp}^2 + \frac{c_0\tau}{4c_3\kappa^2}\fro{\dzt}^2\op{\tz}^2
\end{aligned}
\end{equation}
for any constant $c_3$ to be specified later. Then 
\begin{equation}
\begin{aligned}
\bI_3\leq \left(\frac{\lambda_n}{2\op{\tz}^2}+ \frac{c_0\tau}{4c_3\kappa^2}\right) e_t + c_3\fro{\sigt-\sigp}^2
\end{aligned}
\end{equation}
By the assumption that $\op{\tz}^2\geq C_0\kappa^2\lambda_n/\tau$ for sufficiently large constant $C_0$, 
\begin{equation}
\bI_3\leq \left(\frac{\tau}{2C_0\kappa^2}+ \frac{c_0\tau}{4c_3\kappa^2}\right) e_t + c_3\fro{\sigt-\sigp}^2
\label{nonconvex-I4}
\end{equation}
By basically inequalities, 
\begin{equation}
\begin{aligned}
I_4 &= |\inner{\popt,\widebar{G}}| = |\inner{\sigt - \sigp, \gbar}|\leq \fro{\sigt - \sigp}\fro{\gbar} \\
&\leq c_4\fro{\sigt - \sigp}^2 + \frac{1}{4c_4}\fro{\gbar}^2
\end{aligned}
\end{equation}
for any constant $c_4$ to be specified later. The final step is to control $\bI_5$ by upper bounding its three terms separately, 
\begin{equation}
\begin{aligned}
\fro{\samt \zt}^2&=\fro{\left(\samt-\popt\right) \zt+\popt \zt}^2\\
&\leq 2\Big( \fro{(\samt-\popt)\zt}^2 +\fro{\popt\zt}^2 \Big)\\
&\leq 2\Big( \fro{(\sigp-A)\zt}^2 +\fro{(\sigt-\sigp)\zt}^2 \Big)\\
&\leq 2\Big( \op{\sigp-A}^2\fro{\zt}^2 +\fro{\sigt-\sigp}^2\op{\zt}^2 \Big)\\
&\leq 2\Big( \frac{\lambda_n^2}{4}\fro{\zt}^2 + \fro{\sigt-\sigp}^2\fro{\dallt}^2 \Big)
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
\|\samt \one\|^2&=\left\|\left(\samt-\popt\right) \one+\popt \one\right\|^2\\
&\leq 2\Big( \vnorm{\left(\samt-\popt\right)\one}^2 +\|\popt\one\|^2 \Big)\\
&\leq 2\Big( \vnorm{(\sigp-A)\one}^2 +\vnorm{(\sigt-\sigp)\one}^2 \Big)\\
&\leq 2n\Big(\frac{\lambda_n^2}{4} +\fro{\sigt-\sigp}^2\Big)
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
\inner{\popt, \bX}^2&=\Big(\inner{\samt-\popt, \bX}+\inner{\popt, \bX}\Big)^2\\
&\leq 2\Big(\inner{\sigp-A, \bX}^2+\inner{\sigt-\sigp, \bX}^2\Big)\\
&\leq  2\Big(\lambda_n^2 k\fro{X}^2+\fro{\sigt-\sigp}^2\fro{X}^2\Big)
\end{aligned}
\end{equation}
When $\text{dist}(\zt, \tz)\leq c\op{\tz}$, adding these inequalities will yield
\begin{equation}
\begin{aligned}
\bI_5&\leq 2\left(\frac{\op{\zt}^2}{\op{\tz}^2} \left(\lambda_n^2k/4 + \fro{\dallt}^2/16\right)+\lambda_n^2/8 + \lambda_n^2 k/4+ 3\fro{\dallt}^2/64\right) 
\end{aligned}
\end{equation}
By the assumption that $\fro{\dzt}\leq \frac{c_0\tau}{\kappa^2}\op{\tz}$ for some sufficiently small $c_0$, when $(1+\frac{c_0\tau}{\kappa^2})^2\leq 2$, 
\begin{equation}
\begin{aligned}
\bI_5&\leq C_5 \left(\lambda_n^2k + \fro{\sigt-\sigp}^2\right)
\end{aligned}
\label{nonconvex-I4}
\end{equation}
Combine \eqref{nonconvex-I1}, \eqref{nonconvex-I2}, \eqref{nonconvex-I3} and \eqref{nonconvex-I4} into \eqref{nonconvex-obj},
\begin{equation}
\begin{aligned}
e_{t+1}&\leq e_t-\eta\left(\frac{2(\sqrt{2}-1)}{\kappa^2}\left(\frac{(1-c_1)\tau}{4\tau + 1} - c_2\right) -  \frac{\tau}{2C_0\kappa^2} - \frac{c_0\tau}{4c_3\kappa^2}\right)e_t + \eta \left(C_1 + \frac{1}{4c_4}\right)\fro{\gbar}^2	 \\
& \quad - \left(\frac{1}{\tau + 1/4} - c_3 - c_4 - C_5\eta\right)\fro{\sigt-\sigp}^2 + \eta\frac{C_2}{4c_2}\lambda_n^2k + \eta^2C_5\lambda_n^2k 
\end{aligned}
\end{equation}
where $c_2, c_3, c_4$ are arbitrary constants, $c_0$ is a sufficiently small constant, and $C_0$ is a sufficiently large constant. Choose $c_2 = c\tau$ and $c_3, c_4, \eta$ small enough such that 
\begin{equation}
\begin{gathered}
2(\sqrt{2}-1)\left(\frac{(1-c_1)\tau}{4\tau + 1} - c_2\right) -  \frac{\tau}{2C_0} - \frac{c_0\tau}{4c_3}> 0\\
		\frac{1}{\tau + 1/4} - c_3 - c_4 - C_5\eta \geq 0,
\end{gathered}
\end{equation}
then there exist constants $\rho , C > 0$
\begin{equation}
\begin{aligned}
e_{t+1}&\leq \left(1- \frac{\eta\tau}{\kappa^2}\rho\right)e_t + \eta C \left(\fro{\gbar}^2 + \frac{\lambda_n^2k}{\tau}\right)  
\end{aligned}
\end{equation}
\end{proof}


\begin{lemma}
For any given constant $c_0$, if $\lambda_n\geq \op{A-P}$, $| \langle \bA-\bP, \bX \rangle | \leq \lambda_n\sqrt{k}\fro{X}$, $e_0\leq c_0^2\tau^2/4\kappa_{\tz}^4\op{\tz}^4$ and $\op{\tz}^2\geq C_1\kappa_{\tz}^2\lambda_n/\tau\max\left\{\sqrt{\eta\fro{G}^2/\lambda_n^2}, \sqrt{\eta k/\tau}, 1\right\}$ for sufficiently large constant $C_1$, then under Assumption~\ref{assump:srank}, for all $t\geq 0$, 
\begin{equation}
\fro{\dzt}\leq \frac{c_0\tau}{\kappa_{\tz}^2}\op{\tz} .
\end{equation}
\label{lemma-nonconvex-2}
\end{lemma}
\begin{proof}
	We prove this by induction. For the base case, 
\begin{equation}
\begin{aligned}
\fro{\Delta_{\bZ^0}}\leq \left(\frac{e_0}{\op{\tz}^2}\right)^{\frac{1}{2}}\leq \left(\frac{c_0^2\tau^2}{4\kappa^4}\op{\tz}^2\right)^\frac{1}{2}=\frac{c_0\tau}{2\kappa^2}\op{\tz}\leq \frac{c_0\tau}{\kappa^2}\op{\tz}
\end{aligned}
\end{equation}
Suppose the claim is true for all $t\leq t_0$, by Lemma~\ref{lemma-nonconvex-1}, 
\begin{equation}
\begin{aligned}
e_{t_0+1}&\leq \left(1-\frac{\eta\tau}{\kappa^2}\rho\right)^{t_0}e_0 + \eta C \left(\fro{\gbar}^2 + \frac{\lambda_n^2k}{\tau}\right)  \\
&\leq e_0 + \eta C \left(\fro{\gbar}^2 + \frac{\lambda_n^2k}{\tau}\right)\\  
&\leq \frac{c_0^2\tau^2}{4\kappa^4}\op{\tz}^4 + \eta C \left(\fro{\gbar}^2 + \frac{\lambda_n^2k}{\tau}\right)\\
&=\frac{c_0^2\tau^2}{\kappa^4}\op{\tz}^4  \left(\frac{1}{4}+ \eta\frac{C\lambda_n^2\kappa^4}{c_0^2\tau^2\op{\tz}^4}\left(\frac{\fro{\gbar}^2}{\lambda_n^2} + \frac{k}{\tau}\right)\right)\\
&\leq \frac{c_0^2\tau^2}{\kappa^4}\op{\tz}^4  \left(\frac{1}{4}+ \frac{C}{c_0^2C_1^2}\right)
\end{aligned}
\end{equation}
Choosing $C_1$ large enough such that $C_1^2\geq  \frac{4C}{3c_0^2}$, then
\begin{equation}
e_{t_0+1}\leq \frac{c_0^2\tau^2}{\kappa^4}\op{\tz}^4  
\end{equation}
and therefore, 
\begin{equation}
\fro{\Delta_{\bZ^{t_0+1}}}\leq \left(\frac{e_{t_0+1}}{\op{\tz}^2}\right)^{\frac{1}{2}}\leq \frac{c_0\tau}{\kappa^2}\op{\tz}
\end{equation}
\end{proof}
